High Resolution Point Clouds from mmWave Radar

This paper explores a machine learning approach for generating high resolution point clouds from a single-chip mmWave radar. Unlike lidar and vision-based systems, mmWave radar can operate in harsh environments and see through occlusions like smoke, fog, and dust. Unfortunately, current mmWave processing techniques offer poor spatial resolution compared to lidar point clouds. This paper presents RadarHD, an end-to-end neural network that constructs lidar-like point clouds from low resolution radar input. Enhancing radar images is challenging due to the presence of specular and spurious reflections. Radar data also doesn't map well to traditional image processing techniques due to the signal's sinc-like spreading pattern. We overcome these challenges by training RadarHD on a large volume of raw I/Q radar data paired with lidar point clouds across diverse indoor settings. Our experiments show the ability to generate rich point clouds even in scenes unobserved during training and in the presence of heavy smoke occlusion. Further, RadarHD's point clouds are high-quality enough to work with existing lidar odometry and mapping workflows.

==> interpretability.tex <==
\section{Model Interpretability} \label{sec:interpret}


Our network outputs a general-purpose high resolution image that can be used for odometry, mapping, and other applications. One of the key benefits of such a general-purpose representation rather than end-to-end odometry or mapping ML pipelines is the ability to debug when something goes wrong. For example, if the high resolution image is not accurate for a particular environment, we expect the odometry and mapping to have errors. However, discovering what went wrong merely using odometry output from the network can be challenging in an end-to-end odometry pipeline. 

We now focus on the interpretability of our model. In machine learning literature, attribution techniques have been used to understand what different network layers learn. For example, convolutional networks for image classification have been shown to capture low-level information in the earlier layers and higher-level information in deeper layers \cite{yosinski2015understanding}. Beyond this, attribution techniques have been used for understanding the influence of input, data distribution, and robustness to noise \cite{simonyan2013deep,goodfellow2014explaining}. For our model, we specifically look at the influence of input and layer attributions. 

\subsection{Input Attribution}
Input attribution assigns an importance score to different features in the input, in our case, different pixels of the input radar image. Of the available input attribution techniques, we use Saliency \cite{simonyan2013deep,kokhlikyan2020captum}. Intuitively, for a simple linear model ($w^{T}x+b$), the magnitude of weights $w$ decide which elements of $x$ are important. Saliency extends this to complicated non-linear models, such as our network. Given an input image, a trained model, and an output pixel of interest, Saliency computes the importance score for each individual input pixel. In other words, the Saliency score represents how much an input pixel matters in generating the output pixel. 

Fig. \ref{fig:saliency} shows the Saliency scores of 5 different output pixels of interest marked with colored $\star$. The Saliency score is of the same shape as the input as it is computed for each input pixel. We highlight a few key takeaways of this analysis:


\begin{figure*}[!htb]
\centering
\includegraphics[width=\textwidth]{figures/layer_attribution.pdf}
\vspace*{-0.3in}
\caption{Layer Attribution: This figure shows the layer attributions marked in green at 5 filters at the bottom two resolution levels of \name. The green values show which input pixels matter in predicting white pixels in the output. Clearly, we can see major objects in the environment (shown in colored boxes on the left) triggering the filter attributions on the right. Thus, our model declutters and captures the semantic understanding of the scene.}
\vspace*{-0.2in}
\label{fig:layer_attribution}
\end{figure*}


\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item \textcolor{red}{$\star$}: For inferring pixels which are not occupied in the output ground truth, the model learns to ignore all input pixels and not use any information. Intuitively, we expect the model only to use input pixels when the output pixel of interest is occupied. This result matches our intuition.
    \item \textcolor{mycyan}{$\star$} \textcolor{mypink}{$\star$} \textcolor{mygreen}{$\star$}: For inferring pixels which are occupied in the ground truth, we see that the input pixels used are in the same local neighborhood as the output pixel. For \textcolor{mycyan}{$\star$} \textcolor{mypink}{$\star$} and \textcolor{mygreen}{$\star$}, we accordingly see input pixels in the right bottom corner, center, and top center respectively to be marked as useful. We also note that the input pixels used tend to occupy local 2D regions. This could refer to the process of the model learning \textit{sinc-like} patterns and using all the sidelobes to un-distort the input image.
    \item \textcolor{myorange}{$\star$}: Sometimes even for inferring pixels which are not occupied, we see that certain input pixels in the neighborhood are used. This implies that the structure of the scene in the input image (unlike images used in training) required using all nearby pixels to avoid showing a false output.
\end{itemize}

Overall, we find that input attribution shows us that the locality of input pixels used are indeed pixels relevant to the output. 



\subsection{Layer Attribution}
Layer attribution seeks to understand what is learned by each layer in the model. Recall that our entire network architecture was designed to ensure that the encoder captures the radar artifacts and achieves a semantic understanding while the decoder uses this understanding to perform the upsampling. Here, we focus on obtaining the semantic knowledge of the scene that the encoder captures from noisy input.


Our objective is to study the activations of different convolutional filters, especially in the encoder. We use Layer Conductances \cite{kokhlikyan2020captum,dhamdhere2018important,shrikumar2018computationally}, a technique for layer attribution. The output \textit{attribution} is a 0 to 1 image, one for each filter, with dimensions being the height and width of the filter. Values closer to 1 mark filter weights which are important. As we move lower down the encoder, the filter sizes become smaller and smaller. For sizes smaller than the input dimensions, we upsample the attribution and overlay it on the input image, as shown in Fig. \ref{fig:layer_attribution}. Note that attributions are slightly different from activations in the sense that they capture the activations that matter in inferring a particular region of output pixels. In our case, we use it to look for patterns across filters for generating the white pixels in the output image. We would like to highlight the following key takeaways after studying all 1472 (64+128+256+512+512) terminal convolution filters at each of the 5 "resolution levels" in the encoder (see Fig. \ref{fig:layer_attribution}).

\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item We find that the attributions across different filters are mostly sparse, i.e. contain mostly 0s. This is characteristic of convolutional layer-based encoder networks \cite{yosinski2015understanding}. For typical input data as shown in Fig. \ref{fig:layer_attribution}, we see 10, 26, 68, 8, and 4 filters at each resolution level, respectively, to contain non-zero attribution. This shows that few filters contribute to generating the white pixels. We also observe that the number of total activations is denser than attributions. This shows that apart from the few filters mentioned above that contribute to the white pixels, many other filters do get activated and contribute to the black pixels.
    
    \item Next, we look at the non-zero filter attributions, especially at the bottom-most two resolution levels, which typically capture high-level information \cite{cnn_tut}. Five filter attributions from the bottom layers are overlaid on the input image in Fig.  \ref{fig:layer_attribution}. Our first point to note is that the attributions are significantly less noisy in contrast to the input image. This shows that the encoder does declutter the scene and eliminate the artifacts. In comparison to the ground truth, all important and true reflections in the scene are identified in their correct positions across the five attributions. This tells us that the semantic understanding as interpreted from these attributions accurately represents the real world devoid of radar artifacts. Also, most importantly, because this encoder captures the semantic information, we believe the encoder design can be reused for several other radar tasks beyond super resolution, such as object detection and classification, to name a few. 
\end{itemize}


